Modeling Price Elasticity for Occupancy Prediction in Hotel Dynamic Pricing

Demand estimation plays an important role in dynamic pricing where the optimal price can be obtained via maximizing the revenue based on the demand curve. In online hotel booking platform, the demand or occupancy of rooms varies across room-types and changes over time, and thus it is challenging to get an accurate occupancy estimate. In this paper, we propose a novel hotel demand function that explicitly models the price elasticity of demand for occupancy prediction, and design a price elasticity prediction model to learn the dynamic price elasticity coefficient from a variety of affecting factors. Our model is composed of carefully designed elasticity learning modules to alleviate the endogeneity problem, and trained in a multi-task framework to tackle the data sparseness. We conduct comprehensive experiments on real-world datasets and validate the superiority of our method over the state-of-the-art baselines for both occupancy prediction and dynamic pricing.

==> sec-PCNet.tex <==
\section{PCNet}
\label{sec:pcnet}
% In this section, we present the proposed method extensively. Firstly, we give an overview of the proposed PCNet. Then, we introduce the submodules of PCNet in detail. Finally, we describe the training settings.

\begin{figure*}[htbp]
\centering
\subfigure[The Popularity and Competitiveness aware neural Network (PCNet).]{
\begin{minipage}[t]{0.65\textwidth}
\centering
\includegraphics[scale=0.75]{framework.eps}
% \caption{fig1}
\end{minipage}%
}%
\hspace{2mm}
\subfigure[Selector Block (SB).]{
\begin{minipage}[t]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{selectblo.eps}
% \caption{fig2}
\end{minipage}%
}%
\centering
\caption{The proposed PCNet for occupancy prediction, where $\oplus$ denotes the concatenation. The input includes two parts: the first part includes static and context features of $rid$ and $rid$ group, which is fed into the network as $V_{c}$ by embedding layer. The other is the output of sub-modules, such as $V_{i}$, $V_{e}$ and $V_{l}$.
% internal competitive vector $V_{i}$, which is generated by ICM. The third part is external competitive vector $V_{e}$, which is generated by ECM. The fourth part is long short-term popularity vector $V_{l}$, which is generated by LSPM.
}
\label{PCNet}
\end{figure*}

The architecture of PCNet is illustrated in Fig. \ref{PCNet}. The model mainly consists of four modules: internal competitive representation module captures the hotel competitiveness in similar hotels, external competitive representation module obtains the hotel competitiveness in other booking platforms, long short-term popularity representation module captures the long short-term hotel popularity, and multi-task occupancy prediction module alleviates the data sparsity on occupancy prediction to price hotels more precisely.

\subsection{Competitive Representation Module}
The overall hotel booking demand in a certain area is unchangeable during a certain time. Therefore, when users decide which hotel to book, they always pay a lot attention to the following two key points:
\begin{itemize}
\item Internal competitiveness: the metric of hotel price-performance ratio in similar hotels with the same booking platform.
\item External competitiveness: the metric of price superiority of hotel on different booking platforms.
\end{itemize}
\subsubsection{Internal Competitive Representation Module}
% In this section, we discuss the representation of internal competitiveness.
The occupancy of a hotel is not only related to the price and quality, but also related to the surrounding similar hotels. Specifically, the price of other hotels in same area can affect the price elasticity and supply-demand relationship of the target hotel. As shown in Fig. \ref{submodule}, ICM consists of three components. First, a similar $rid$ group is obtained by spectral clustering \cite{ct3}, which is mainly considered the location, room type, hotel star and price of the $rid$, and evaluated by manual sampling. Second, a weighted undirected graph of $rid$ and historical booking price is constructed in each group, where the weight is the reservation nights of the $rid$ on the corresponding price, and we apply metapath2vec \cite{ct4} to get the latent embedding of $rid$ and price in group. Finally, the differential features (such as room size, decoration time, evaluation score, etc.) in a group are transformed into low-dimensional vector by embedding layer to capture the quality representation. The embeddings of $rid$ and quality are concatenated as internal competitive representation.
% Specifically, for the new price not contained in the training sample, the average values of two nearest neighbor embedding are calculated to represent the embedding of new price.
\subsubsection{External Competitive Representation Module}
The crucial factor that users consider when comparing different booking platforms is price, this section mainly captures the price competitiveness of hotel. As shown in Fig. \ref{submodule}, the external competitive representation module mainly adopts FM to obtain cross combination of different features and output the concatenation as external competitive representation. The input of ECM includes hotel price in other booking platform, statistical variables of price and marketing information. It is empirical to combine the power of factorization machines (FM) \cite{ct16} for interactive learning of features, which captures order-2 feature interactions much more effectively when the dataset is sparse. Limited by technology and security, the way to obtain hotel prices on other platforms is relatively single, both the stability of data acquisition and matching rate is not robust. Therefore, we introduce a selector block to filter the harmful noise from the data source.

\begin{figure*}[htbp]
\centering
\subfigure[Long Short-term Popularity representation Module (LSPM).]{
\begin{minipage}[t]{0.5\textwidth}
\centering
\includegraphics[width=\textwidth]{LSPM.eps}
% \caption{fig1}
\end{minipage}%
}%
\hspace{5mm}
\subfigure[Internal Competitive representation Module (ICM).]{
\begin{minipage}[t]{0.25\textwidth}
\centering
\includegraphics[width=\textwidth]{ICM.eps}
% \caption{fig2}
\end{minipage}%
}%
\hspace{5mm}
\subfigure[External Competitive representation Module (ECM).]{
\begin{minipage}[t]{0.15\textwidth}
\centering
\includegraphics[width=\textwidth]{ECRW.eps}
% \caption{fig2}
\end{minipage}
}%

\centering
\caption{The sub-modules of PCNet. LSPM, ICM and ECM are developed to capture the long short-term popularity, hotel competitiveness in similar hotels and hotel competitiveness in other booking platforms respectively.}
\label{submodule}
\end{figure*}


\subsection{Long Short-term Popularity Representation Module}
As mentioned above, hotel occupancy is related to the competitiveness of hotel. Meanwhile, the sales of hotels are obviously affected by the market trend and seasons. For example, hotspring hotels are popular in winter, and hotels that around the scenic spot are in short supply on holidays. Travel activities subject to quite strong seasonal variation. Moreover, special events also cause a surge in demand for certain nights in the region where the event is held. We uniformly define this characteristic as long short-term popularity. As illustrated in Fig. \ref{submodule}, the output of LSPM is the concatenation of long-term popularity representation and short-term popularity representation.

\subsubsection{Short-term Popularity Representation}
The short-term sequences consists of ipvuv, search uv, sale price, booking price and hotel occupancy in the last month, which represent the recently popularity of the hotel. For example, the sequence of ipvuv indicates the number of users who click the hotel and the sequence of search uv shows the number of users searching for the hotel. As shown in Fig. \ref{submodule}, 
one-dimensional convolution with different kernel size is applied to 
% GRU \cite{ct6} is applied to capture the recently popularity trend of the hotel by fusing the multiple sequences. In addition, we adopt one-dimensional convolution to 
capture the combined features of multiple sequences, which can obtain local combined trend patterns of hotel. The concatenation of local combined trend in different time spans is used for short-term popularity $H_{s}$.
\subsubsection{Long-term Popularity Representation}
To capture the long-term popularity, the proportion of sales, pv, ipvuv and search uv in all hotels of a region are divided into three temporal granularity of sequences (day, week, month). Let $s_{wi}$ be the proportion of variable $s$ for day $w$ of the week and weeks number $i$ in a half year, $s_{mj}$ be the proportion of variable $s$ for each month $m$ and years number $j$ in recent 3 years, and $s_{dk}$ be the proportion of variable $s$ for each day $d$ and months number $k$ in recent year. Then the input sequences can be given as:
\begin{equation}
s_{w} = \sum\limits_{i}{s_{wi}}
\end{equation}
\begin{equation}
s_{m} = \sum\limits_{j}{s_{mj}}
\end{equation}
\begin{equation}
s_{d} = \sum\limits_{k}{s_{dk}}
\end{equation}
Due to the popularity of different $rid$s varies greatly in different periods, the historical date is transformed into low-dimensional dense features by embedding layer, and the context date is input into different embedding layer. The embedding of long-term sequence, historical date and context date in temporal granularity $t$ can be represented as $x_{ts}$, $x_{th}$ and $x_{tc}$, respectively. In order to obtain the long-term popularity with different temporal granularity, the time-aware attention is utilized to activate the weight of diverse trends to capture the timeliness of each trend. Specifically, the attention function takes the context time, the historical time and long-term sequence embeddings as the query, key and value respectively. We compute the final long-term popularity representation $H_{l}$ as:
\begin{equation}
H_{l} = Attention(x_{ts}, x_{th}, x_{tc}) = x_{ts}softmax(x_{th}x_{tc}^{T})
\end{equation}
where $Attention$ denotes the attention function.

\subsection{Multi-task Occupancy Prediction Module}
According to Eq. \ref{sales_eq}, PCNet is designed to learn the price elasticity term and natural growth term that affect the occupancy. However, the sparsity of hotel reservation data will affect the learning ability of the method, and the daily occupancy of a single rid fluctuates greatly, resulting in inaccurate learning of natural growth terms. The distribution of reservation days of $rid$ and $shid$ in recent months is illustrated in Fig. \ref{days}. Inspired by multi-task learning \cite{ct34,ct35}, we alleviate the data sparsity by learning occupancy of $rid$ and $rid$ group together to improve the prediction accuracy of $rid$. 

As shown in Fig. \ref{PCNet}, there are multiple objectives to model different prediction targets such as price elasticity $W_^{g}$ and natural growth $b_^{g}$ of group in auxiliary task, price elasticity $W_^{r}$ and natural growth $b_^{r}$ of $rid$ in main task. To better exploit correlations between terms in a task, MLP layer are introduced to fuse more abstract representations. Moreover, selector block is applied to alleviate the differentiation and avoid harmful parameter interference, which is defined as:
\begin{equation}
SB(x) = x \otimes sigmoid(Wx+b)
\end{equation} 
where $\otimes$ denotes the hadamard product. Let $V_{c} \in \mathbb{R}^{n \times d_{v}}$ denotes the embedding of static features (such as location, business district, hotel star, etc.) and context features (real-time selling price, competitive selling price, holiday info, etc.), where $n$ is the total number of features and $d_{v}$ is the embedding size. The network input of $rid$ price elasticity, $rid$ natural growth and group task can be depicted by the following equation:
\begin{equation}
Input^{r}_{W} = Concat(V^{r}_{c}, V^{r}_{i}, V^{r'}_{e})
\end{equation}
\begin{equation}
Input^{r}_{b} = Concat(V^{r}_{c}, V^{r}_{l})
\end{equation}
\begin{equation}
Input^{g} = Concat(V^{g}_{c}, V^{g}_{l})
\end{equation}
where $V^{r'}_{e}$ denotes the output of ECM after selector block.
% and can be given as:
% \begin{equation}
% V^{r'}_{e} = SB(V_{e})
% \end{equation}
% which mainly considers the instability of data acquisition, it may bring harmful noise to the learning of the occupancy. The negative features in ECM are filtered out by selector block.

Negative transfer \cite{ct33} is a common phenomenon between different tasks, we observe that improving joint learning efficiency and achieving significant improvement over the corresponding single-task model across all tasks is difficult for hotel. Therefore, we introduce a novel gating network to achieve more efficient information transfer in occupancy prediction, which obtains fusing weights based on the similarity of long short-term popularity of $rid$ and group. Specifically, the formulation of the gating network is:
\begin{equation}
g(x) = x \otimes Sigmoid(SB(V_{l}^{g}) \otimes SB(V_{l}^{r}))
\end{equation}
The gating network takes the similarity of $rid$ and group as the selector
instead of the raw input, as it may provide better information for selecting abstract knowledge extracted in LSPM whose correlation is greater with $rid$ natural growth term.

The objective of PCNet is minimizing the loss $\ell$, which is given as:
\begin{equation}
\ell=\alpha \cdot H_{\theta}^{r}(F(P))+\beta \cdot H_{\theta}^{g}(F(P))
\end{equation}
where $\alpha, \beta$ are hyper-parameters, $H_{\theta}(H(P))$ is huber loss \cite{ct2} and defined as:
\begin{equation}
H_{\theta}(x)=
\begin{cases} 
\frac{1}{2}x^{2},  & |x|\leqslant\theta \\
\theta(|x|-\frac{1}{2}\theta), & |x|>\theta
\end{cases}
\end{equation}
where $\theta\in \mathbb{R}^{+}$.

\subsection{Training}
Considering the interpretability of the pricing result for hotel managers and the accuracy of the average sales $Q_{avg}$ in recently month as the result in occupancy prediction, we define the benchmark sales as $Q_{0}=K\cdot Q_{avg}$, where $K$ is a hyper-parameter introduced to adjust the effect of the price elasticity. In real-life experiments, we often observe that the suggested price is abnormal and unstable, such as overly high or low. Given the upper bound $P_{max}$ and lower bound $P_{min}$ of pricing range, we require that:
\begin{align}
F(P)=K\cdot Q_{avg}\cdot e^{WP}+\frac{b}{P}, \quad \quad     &  -\frac{1}{P_{min}}\leq W \leq -\frac{1}{P_{max}}
\end{align}

In the offline training process, we train the PCNet based on user reservation actions extracted from reservation logs. Each $rid$ group contains 6 $rid$s. Mini-Batches and drop-out units are used to regularize model training. Specifically, first MLP layer in each task contains 2 hidden layers with 512, 256 units respectively and second MLP contains 2 hidden layers with the number of hidden nodes $\{128, 1\}$. The embedding size of hotel features is set as 16. The dimension of hotel-price latent vector is 32. 
% The LSPM contains 2 convolution kernels with the sizes of 64, 32 and a GRU with 64 units respectively. Hyper-parameters are chosen on a global level or on a few important listing cohorts to avoid over-tuning.
The batch size is 512, the dropout rate is 0.2, $K$ is 1.1, $\alpha$ is 1.0 and the $\beta$ is 0.5. We use Adam \cite{ct37} as the optimizer and set the learning rate as 0.001. The experiments are implemented based on Keras \cite{ct32} and trained on GPU.

==> sec-dynamic_pricing.tex <==
\section{Dynamic PRICING SYSTEM}
\label{sec:pricing}
The pricing system (shown in Fig. \ref{overview}) is mainly composed of occupancy prediction model, which outputs the optimal price by occupancy learning when given sale price and the pricing range.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=200 pt]{overview.eps}
  \caption{Overview of the pricing system.}
  \Description{}
  \label{overview}
\end{figure}


\subsection{Problem Definition}
The smallest saleable unit is called $rate$ in Fliggy, which is composed of a certain room type ($rid$) and price policy. $shid$ represents the standard hotel ID. Generally, a standard hotel contains multiple different room types. Let $S=\{shid_{1},shid_{2},shid_{i}...shid_{n}\}$ be a set of hotels, $R=\{rid_{i1},rid_{i2},rid_{ij}...rid_{im}\}$ be the set of room types under hotel $shid_{i}$, the room nights of $shid_{i}$ is the sum of $rid_{im}$ room nights. We set the optimal price $P^{*}$ for each room type.

\begin{table}[htbp]
  \caption{Notations.}
  \label{tab:notation}
  \begin{tabular}{cll}
    \toprule
     Notation&Description\\
    \midrule
    $shid$ and $rid$ & hotel ID and room type ID\\
    % $Q$ and $Q_{0}$ & room nights of prediction and benchmark\\
    $P_{max}$ and $P_{min}$ & the upper bound and lower bound of price\\
    $P$ and $P^{*}$ & hotel price and optimal price\\
    $W$ and $b$ & model parameters\\
    $E$ and $Q_{0}$ & hotel revenue and the benchmark sales\\
    $K$, $\alpha$ and $\beta$& hyper-parameters\\
    $V^{g}_{m}$ and $V^{r}_{m}$ & embedding of group and rid for module $m$\\
    % $V^{'}$ & embedding vector after selector block\\
    $s_{w}$, $s_{m}$ and $s_{d}$ & input sequence of week, month and day\\
  \bottomrule
\end{tabular}
\end{table}

\subsection{Occupancy Prediction}
% when other variables are fixed and affect the hotel sales only by pricing,
In demand estimation, the sales consist of the natural growth of hotel sales, and the growth affected by price that we called price elasticity. Considering the inverse correlation between price and sales, and the impact of price is significant in all the variables that affect sales. We assume that the price elasticity obeys the exponential distribution, and the demand function $F(P)$ is given as:
\begin{equation}
\label{sales_eq}
F(P)=Q_{0}\cdot e^{WP}+\frac{b}{P}
\end{equation}
% , which is affected by abnormal prices (overly high or low)
where $W<0$, $P$ and $Q_{0}$ represent the selling price and the benchmark sales respectively. The formula consists of two terms, the first represents the price elasticity and the other represents the natural growth of hotel sales. Further, the hotel occupancy with selling price $P$ can be written as $F(P)/iv$, where $iv$ represent the hotel inventory. We develop a framework PCNet to predict the occupancy of all room types based on Eq. \ref{sales_eq}, which we will discuss in more detail in Sec. \ref{model}. Compared with the traditional occupancy prediction model \cite{ct24}, we introduce the explicit impact of price on the prediction, which makes the occupancy prediction more accurate and the pricing more flexible.

\subsection{Pricing Strategy}
Researches of dynamic pricing often focus on demand estimation \cite{ct15}. A demand function can be obtained by tracking how demand varies with respect to price for a large number of identical products, and the optimal price $P^{*}$ can be obtained via maximizing the expected revenue based on the demand function.
\begin{equation}
P^{*}=\mathop{argmax}\limits_{P} P\cdot F(P)
\end{equation}
% In the Fliggy pricing problem, the hotels are homogeneous products, which enables the model to learn the supply-demand relationship of the target hotel by other similar hotels, 
% The time-varying demand function $F(P)$ fit the formula \ref{sales_eq} proposed in the previous section. 
The expected revenue $E$ can be defined as
\begin{equation}
E=P\cdot Q_{0}\cdot e^{WP}+b
\end{equation}
It is a concave function with a global maximum. We can express directional derivative as 
\begin{equation}
\frac{\partial E}{\partial P}=(1+PW)\cdot Q_{0}\cdot e^{WP}
\end{equation}
And the optimal price $P^{*}$ is given by:
\begin{equation}
P^{*}=-\frac{1}{W}
\end{equation}

Our pricing strategy aims to predict the hotel occupancy and obtain the optimal price by a end-to-end deep model.

==> sec-expt.tex <==
\section{EXPERIMENTS}
\label{sec:expt}
In this section, we conduct extensive experiments on two real-world datasets to answer three questions: (\textbf{Q1}) How does the PEM model perform in occupancy prediction? (\textbf{Q2}) How does the proposed elastic demand function work in dynamic pricing? (\textbf{Q3}) How do different modules and losses contribute to the performance?
%R4: How does the proposed method perform in live hotel reservation services? 
% In this section, firstly, we describe the datasets, comparing methods and evaluation metrics. Secondly, we introduce the state-of-the-art prediction methods of occupancy prediction and dynamic pricing strategy. Finally we evaluate the performance of pricing strategy and analyze what the experimental results indicate.

\subsection{Experimental Settings}
\subsubsection{Datasets.}
% As there is no public datasets for hotel pricing, 
We construct two datasets by the hotel reservation logs collected from Fliggy\footnote{\url{www.fliggy.com}}, which is one of the most popular online travel platform in China.
% Fliggy is one of the most popular online travel platform in China serving tens of millions of users with million-scaled travel-related items such as hotels, tickets. 
%We construct the training set on $12727$ hotels that have reservation records from 2020-12-17 to 2021-01-16, containing the basic features, historical transaction statistics in the past one month  
In particular, \emph{Dataset-H} and \emph{Dataset-L} are based on the hotel reservation data in a high-booking season from 2020.12.17 to 2021.01.23 and a low-booking season from 2021.03.11 to 2022.04.17, respectively. 
In each dataset, the reservations in the first 30 days are employed as the training set to predict the occupancy and suggest price for the next 7 days. 
The details of the datasets are summarized in Table~\ref{tbl:datasets}.  
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\center
\small
\caption{Summary of datasets.}
\vspace{-3mm}
\addtolength{\tabcolsep}{-0.6mm}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{}c|rrr|rrr@{}}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Datasets}} & \multicolumn{3}{c|}{Training}                                           & \multicolumn{3}{c}{Testing} \\
\cline{2-7}
\multicolumn{1}{c|}{}                                                                       & \# hotels & \# rooms & \# reservations &   \# hotels  & \# rooms & \# reservations \\
\cline{1-7}
\begin{tabular}[c]{@{}l@{}}Dataset-H \end{tabular}                                         & 12,727 &  16,676   & 712K &      7,859   &  10,023       &      222K        \\
% \hline
   \begin{tabular}[c]{@{}l@{}}Dataset-L \end{tabular}                                     & 11,556 &   14,801 & 834K    & 9,533        & 12,804        &     169K             \\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\label{tbl:datasets}
\end{table}

%one of the most popular online booking platform that provides hotel reservation services

\subsubsection{Baselines.}
We compare our method with two groups of baselines, \ie, occupancy prediction and dynamic pricing.

% \sstitle{Occupancy prediction approaches}:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Moving Average method (MA)} \cite{warren2017occupancy} uses the average occupancy of past $n$ observations to forecast the next occupancy. {\color{red} n=? in experiment}
%     \item \textbf{Single exponential smoothing (SES)} \cite{warren2017occupancy} weights the past $n$ observations with exponentially decreasing weights to forecast the next occupancy.
%     \item \textbf{Prophet} \cite{forecasting2017} is a time series forecasting model designed to handle the common features of business time series including seasonalities, trend changes, and holiday effects.
%     %\item \textbf{Seq2seq~\cite{sequence2seq2014}} that learns to model the dynamics of time series and regress the label.
%     \item \textbf{GBDT} \cite{stochastic1999} is an additive regression model that gives the prediction in the form of an ensemble of decision trees. We use the algorithm implemented by eXtreme Gradient Boosting (XGBoost) ~\cite{chen2015xgboost}.
%     \item \textbf{DeepFM+Seq2seq} \cite{deeplearningHotel2019} is a sequence learning model for occupancy prediction which integrates DeepFM and Seq2Seq model to learn the interaction among different features in the sequence and regress the future occupancy.
% \end{itemize}

\stitle{Occupancy prediction approaches.}
%(1) \emph{Moving Average method (MA)} \cite{warren2017occupancy} uses the average occupancy of past $n$ observations to forecast the next occupancy.
(1) \emph{GBDT} \cite{stochastic1999} is an additive regression model that gives the prediction in the form of an ensemble of decision trees. 
(2) \emph{Seasonal Autoregressive Integrated Moving Average (SARIMA)} \cite{warren2017occupancy}  combines autoregressive model with moving average to model time series exhibiting seasonality.
%(2) \emph{Single exponential smoothing (SES)} \cite{warren2017occupancy} weights the past $n$ observations with exponentially decreasing weights to forecast the next occupancy.
%(2) \emph{Prophet} \cite{forecasting2017} is a time series forecasting model designed to handle the common features of business time series including seasonalities, trend changes, and holiday effects.
(3) \emph{DeepFM+Seq2seq} \cite{deeplearningHotel2019} is a sequence learning model for occupancy prediction which integrates DeepFM and Seq2Seq model to learn the interaction among different features in the sequence and regress the future occupancy.
(4) \emph{DeepAR} \cite{deepAR2019} is a probabilistic time series forecasting method based on auto-regressive recurrent network.
(5) \emph{TFT} \cite{temporal2020} combines recurrent layers with self-attention layers \cite{vaswani2017attention} to learn temporal relationships at different scales. 


% \sstitle{Dynamic pricing approaches:} 
% % We compare our dynamic pricing strategy with a manual pricing strategy and the state-of-the-art pricing model in hotel industry.
% \begin{itemize}[leftmargin=*]
% \item \textbf{Manual pricing} relies on a set of rules specified by domain experts to set the base price and make adjustment based on the predicted occupancy, and it is currently used in Fliggy's hotel reservation service.
% \item \textbf{DNN-based pricing} \cite{deeplearningHotel2019} adopts a DNN model to regress the suggested price for a certain room at a specific date from the input features.
% \item \textbf{Airbnb pricing} \cite{customized2018} uses a customized regression model to suggest the price \wrt\ the booking probability for Airbnb listing-nights and applies personalized logic to optimize the suggestion.
% \end{itemize}

\stitle{Dynamic pricing approaches.}
%(1) \emph{Manual pricing} relies on a set of rules specified by domain experts to set the base price and make adjustment based on the predicted occupancy, and it is currently used in Fliggy's hotel reservation service.
(1) \emph{DNN-based pricing} \cite{deeplearningHotel2019} adopts a DNN model to regress the suggested price for a certain room at a specific date from the input features.
(2) \emph{Airbnb pricing} \cite{customized2018} uses a customized regression model to suggest the price \wrt\ the booking probability for Airbnb listing-nights and applies personalized logic to optimize the suggestion.

Among these baselines, DeepFM+Seq2Seq and TFT are the state-of-the-art methods for occupancy prediction and general time series forecasting respectively. DNN-based pricing and Airbnb pricing are the only published work in dynamic hotel pricing.

\subsubsection{Implementation details.}
% 
Our proposed PEM contains two fully-connected layers with 256 and 128 units, respectively. The embedding size of all features is set to 16. %The dimension of $\mathbf{c}_r^t$ and $\mathbf{m}_r^t$ is set to 32. 
The multi-sequence fusion model contains three convolution kernels (sizes: 64, 128, 64) and a two-layer Bi-GRU module (number of units: 64, 32). {For training, the batch size is set to 512,} dropout rate is 0.2, $\delta=1.0$ and $\lambda=0.9$. %\zemin{Our model is implemented based on Keras \cite{keras} and trained with GPU. Adam optimizer with learning rate 0.001 is used to update parameters.} 
For GBDT, we use the algorithm implemented by eXtreme Gradient Boosting (XGBoost) \cite{chen2015xgboost} where the number of trees and the max tree length in GBDT is set to 500 and 6 respectively; For SARIMA, we adopt the x13-auto-arima version \cite{gomez2000automatic} of the algorithm. The neural network used in DeepAR and TFT is one-layer LSTM \cite{hochreiter1997long} with 40 and 16 hidden cells respectively, number of heads in the multi-head attention layer of TFT is set to 2. The regression module of Airbnb is a three-layer MLP (number of hidden nodes: $128,32,1$). The other parameters are set as suggested in the original papers. %\zeminC{标注蓝色的是可以删掉的}

% our PEM model: stopping criteria: number of iterations; no early stopping; weight decay:采用指数衰减（tf.train.exponential_decay），每20000步按0.9指数衰减; dropout：每个MLP的第一层加上dropout(0.2)；每个dense层都采用batch normalization

%DeepAR:  RNN 中的隐层层数num_layers=1,RNN 中各隐层cell的个数num_cells=40,RNN中cell的类型cell_type=LSTM,RNN中dropout的比例dropout_rate=0.1,对静态分类特征做嵌入时的维度embedding_size=32

%TFT: 特征的embedding_size=16，LSTM的层数=1，attention的head数=2，batch size=256，learning rate=0.01，dropout_rate=0.1，神经网络隐层大小=16

%DNN-based pricing参数：embedding size为16，learning rate=0.01，seq2seq用的序列模型是LSTM

%Airbnb：第一阶段采用GBDT对预定概率建模，将其输入到第二阶段，第二阶段采用airbnb的定制loss，并采用一个3层的MLP（128*32*1）回归预订价格

%For baselines, we follow the settings in the original papers:   

\subsection{Performance Comparison}
%\subsubsection{Occupancy Prediction}
\subsubsection{Evaluation metrics.} 
We adopt two common metrics MAPE and WMAPE \cite{de2016mean,tofallis2015better} for the evaluation of occupancy prediction.
% To evaluate the accuracy of occupancy prediction, we adopt two common metrics MAPE and WMAPE \cite{de2016mean,tofallis2015better}:
\begin{comment}
\begin{itemize}[leftmargin=*]
    \item $MAPE=100/n\times \sum_{i=1}^N |(O_i-\hat{O}_i)/O_i|$ measures the percentage error of the predicted occupancy in relation to the actual values. 
    \item $WMAPE=\sum_{i=1}^N (w_i|O_i-\hat{O_i}|/\sum_{i=1}^N(w_i|O_i|))$ takes into account the importance $w_i$ of each prediction. \fw{how to determine $w_i$} 
\end{itemize}
\end{comment}
For the evaluation of pricing strategy, we adopt the same metrics employed in hotel dynamic pricing \cite{customized2018,deeplearningHotel2019}: PDR, PDP, PIR, PIP and BR. The detailed description of these metrics can be referred to \cite{deeplearningHotel2019}.
%Among which, PDR and BR are the most important metrics in practice. 
%\zemin{PDR (or PIR) measures the degree that the suggested prices are lower (or higher) than the listing prices for non-booked rooms (or booked rooms)}; BR measures the closeness between the suggested prices and the booked prices. \zemin{PDP???}
Generally, BR measures the closeness between the suggested prices and the booked prices, and the other four metrics measures the profit improvement at the suggested prices. In practice, there should be trade-offs for these metrics to increase the overall revenue of the platform and to maintain business trust from hoteliers. 


%lower BR (booking regret) values indicate better price suggestions, while for the other metrics, higher values are better. 


\begin{table}[]
 \caption{Evaluation on occupancy prediction (in percent).}
    \centering
    % \vspace{-3mm} 
    % {\footnotesize Henceforth, the best tabular result is \textbf{bolded} and the runner-up is \underline{underlined}.}
    % \\[2mm] 
    \vspace{-2mm}
    \resizebox{0.86\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c}
    \toprule
   \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Dataset-H} & \multicolumn{2}{c}{Dataset-L} \\
   \cline{2-5}
           &MAPE $\downarrow$ & WMAPE $\downarrow$  &MAPE $\downarrow$ & WMAPE $\downarrow$  \\
         \hline
        % MA & 54.36 & 49.90 & 57.24& 52.17 \\
        
        %  SES &56.57 &57.43 &59.03 &58.91\\
        %  Prophet & 54.37 & 52.88 &56.30 &52.11 \\
          GBDT & 43.83 & 42.57 & 45.80 &46.51\\
          SARIMA & 28.56 & 40.03 & 30.51 & 41.10\\
          DeepFM+Seq2seq & 28.72 & 39.75 & 30.22& 41.13\\
          DeepAR & 28.11 & 39.78 & 30.24 & 40.86\\
          TFT & 27.96 & 39.22 & 30.03 & 40.37\\
          PEM & \textbf{27.88} & \textbf{39.03} & \textbf{29.86} & \textbf{40.21}\\
         \bottomrule
    \end{tabular}
   }
   \vspace{-2mm}
    \label{tbl:occupancy}
\end{table}


% \begin{table}[htbp]
%   \caption{Evaluation on pricing strategy (in percent).}
%   \label{tbl:pricing}
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
%     \toprule
%   \multirow{2}{*}{Method} & \multicolumn{5}{c|}{Dataset-H} & \multicolumn{5}{c}{Dataset-L} \\
%   \cline{2-11}
%           &PDR & PDP  &PIR & PIP& BR & PDR & PDP  &PIR & PIP& BR \\
%          \hline
%           Manual & 95.86 & 63.34 & 14.09& 68.75 &20.0 &75.26 &58.17 &16.18 &29.69 & 15.11\\
%           DNN &60.63 &59.41 &35.85 &37.03& 5.57 &53.95& 53.65&27.83 &28.08 &7.83 \\
%           Airbnb & 60.33 & 59.70& 34.27 &35.82 & 5.49 & 54.83 & 50.34 & 26.95 & 27.80 & 8.08\\
%           PEM & 61.34 & 60.46 &37.88 &38.75 &5.96 & 56.24& 55.47 &30.09 &30.76 &8.46\\
%          \bottomrule
%     \end{tabular}
% }
% \end{table}


\begin{table}[htbp]
  \caption{Evaluation on pricing strategy (in percent).}
  \vspace{-1mm}
  \label{tbl:pricing}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
   \multirow{2}{*}{Method} & \multicolumn{5}{c|}{Dataset-H} & \multicolumn{5}{c}{Dataset-L} \\
   \cline{2-11}
           &PDR $\uparrow$ & PDP $\uparrow$  &PIR $\uparrow$ & PIP $\uparrow$ & BR $\downarrow$ & PDR $\uparrow$ & PDP $\uparrow$  & PIR $\uparrow$ & PIP $\uparrow$ & BR $\downarrow$ \\
         \hline
         % Manual &\textbf{75.3} &\textbf{58.2} &16.2 &29.7 & 15.1 & \textbf{95.9} & \textbf{63.3} & 14.1 & 68.8 &20.0 \\
          DNN &54.0& 53.7&27.8 &28.1 & \ \ \textbf{7.8} &60.6 &59.4 &35.9 &37.0& \ \ 5.6  \\
          Airbnb &54.8 & 50.3 & 27.0 & 27.8 & \ \ {8.1} & 60.3 & 59.7& 34.3 &35.8 & \ \ \textbf{5.5} \\
          PEM & \textbf{56.2}& \textbf{55.5} &\textbf{30.1} &\textbf{30.8} & \ \ 8.5 & \textbf{61.3} & \textbf{60.5} &\textbf{37.9} &\textbf{38.8} & \ \ 6.0 \\
         \bottomrule
    \end{tabular}
}
\vspace{-5mm}
\end{table}


\subsubsection{Results and analysis.}
The comparison of occupancy prediction and dynamic pricing are shown in Tables~\ref{tbl:occupancy} and \ref{tbl:pricing}, respectively.
For occupancy prediction, PEM achieves the best performance in terms of both metrics, which validates the effectiveness of our elastic demand function and the price elasticity prediction model for occupancy forecasting (\textbf{Q1}).
For dynamic pricing, we observe:
1) PEM significantly outperforms DNN and Airbnb on the first four metrics related to revenue improvement. 2) The BR value of PEM is approaching DNN and Airbnb which are designed to directly regress the booking prices. However, for these baselines, the improvement in BR is obtained at the expense of much worse profit gains. In contrast, our PEM model achieves the best trade-offs among these metrics, {demonstrating} the effectiveness of our pricing strategy with elastic demand function (\textbf{Q2}).

%1) Manual pricing strategy obtains the best PDR at the expense of worse PIR and BR, as manual pricing tends to suggest lower prices for promotion; 2) 
%DNN and Airbnb pricing strategies exhibit good performance in BR as they suggest the optimal price by directly regressing the booking prices. However, their performance in other metrics are not so satisfied mainly due to their inaccurate occupancy (or booking probability) estimation. In contrast, our PEM model achieves the best trade-offs among these metrics: it significantly improves DNN and Airbnb on the first four metrics and achieves approaching performance on BR. The results demonstrate the effectiveness of our pricing strategy with elastic demand function (\textbf{Q2}).
We also deploy our model in the live environment of Fliggy hotel booking system and evaluate the platform revenue with Gross Merchandise Volumn (GMV)~\cite{miao2020data}, a metric commonly-used in e-commerce industry. In the online test for two weeks, the PEM model achieves an average of $7.42\%$ improvement in daily GMV compared with a baseline manual pricing strategy. The details of online experiments are omitted due to the space limitation.

%while our method can achieve better trade-off among these metrics (\eg, $61.34\%$ for PDR and $5.96\%$ for BR). PEM also significantly improves the state-of-the-art DNN pricing model in all metrics except from BR. \fw{The reason is...}

\subsection{Ablation Study \textbf{(Q3)}}

\begin{wraptable}{r}{0.38\linewidth}
    \centering
    \vspace{-4mm}
    \renewcommand{\arraystretch}{1.2}
    \addtolength{\tabcolsep}{-3pt}
    % \addtolength{\tabcolsep}{0pt}
  \caption{Ablation study.}
      \label{tbl:ablation}%
    \vspace{-2mm}
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{c|c|c}
    \toprule
        Method & MAPE $\downarrow$ & WMAPE $\downarrow$ \\ \hline
        PEM-C & 29.01 & 40.15 \\ %\hline
        PEM-M & 48.18 & 52.32 \\ %\hline
        PEM-L & 28.39 & 39.81 \\ 
        PEM & \textbf{27.88} & \textbf{39.03} \\ %\hline
        \bottomrule
    \end{tabular}}
     \vspace{-2mm}
\end{wraptable}
We conduct an ablation study to investigate the contribution of each key module and loss. We compare PEM with three variants: 1) PEM-C: without competitiveness representation module; 2) PEM-M: without multi-sequence fusion module; 3) PEM-L: without hotel-level occupancy prediction task.
The experimental results illustrated in Table~\ref{tbl:ablation} verify that all the components and losses are essential, among which the multi-sequence fusion module contributes the most. 
Specifically, on Dataset-H, the accuracy of PEM-C, PEM-M and PEM-L in WMAPE  drops by $2.4\%$, $2.7\%$, $1.3\%$  respectively.
% \begin{table}[]
%     \centering
%      \caption{Ablation study on Dataset-H.}
%     \begin{tabular}{c|c|c}
%     \toprule
%         Method & MAPE (\%) & WMAPE (\%)\\ \hline
%         PEM & 27.88 & 39.03 \\ \hline
%         PEM-C & 29.01 & 40.15 \\ \hline
%         PEM-M & 48.18 & 52.32 \\ \hline
%         PEM-L & 28.39 & 39.81 \\ 
%         \bottomrule
%     \end{tabular}
%     \label{tbl:ablation}
% \end{table}

\begin{comment}
\subsection{Online A/B Test}
With the success in offline experiments, we deploy the PCNet in daily environment with 24000 $rid$s at Fliggy. In the online experiments, the baseline method is GBDT based demand curve adopted in the previous system, and we consider an important metric GMV in online experiments to evaluate the methods:
\begin{equation}
GMV = \sum\limits_{i}^{n}{P_{i}\cdot F(P_{i})}
\end{equation}
where $n$ denotes the $rid$ number. The experiments are conducted from
2021-09-10 to 2021-09-24 and the average improvements are shown in Table \ref{tab:online}. Fig. \ref{online} shows the online results in 15 days. Considering the data confidentiality policy in Alibaba Group, we use ``*'' as the baseline to replace the absolute values at Fliggy online and report the improvements in Table \ref{tab:online} and Fig. \ref{online}. From this result, we find that PCNet has a large improvement at GMV. The GMV is improved by about $11\%$ compared with the previous system. Which verifies the superiority of PCNet on hotel dynamic pricing.


\begin{table}[htbp]
  \caption{Performance improvements in online A/B tests.}
  \label{tab:online}
  \resizebox{\linewidth}{!}{
  \begin{tabular}{c|c|c}
    \toprule
     Metric &\makecell[c]{GBDT based demand curve\\(Baseline)}&PCNet Pricing Strategy\\
    \midrule
    GMV & $*$ & $+11.39\%$\\
  \bottomrule
\end{tabular}
}
\end{table}
\end{comment}




==> sec-intro.tex <==
\section{Introduction}
\label{sec:intro}
Dynamic pricing~\cite{dynamicPricing2015}, which determines the optimal prices of products or services based on the dynamic market demands, has received considerable attention in research~\cite{demand_elasticity2018,mannagementModel2006} and industries~\cite{hotel2004,dynamic_airline2019,comparison2003,customized2018,yang2014matching,roozbehani2010dynamic,deeplearningHotel2019}.
%due to its importance in balancing supply and demand~\cite{roozbehani2010dynamic} and revenue management~\cite{bitran2003overview}.
In online hotel reservation platforms (\eg, booking.com, Fliggy), dynamic pricing is extremely important as similar hotels on the platform compete to share the market demand, and the inventory (\ie, the available rooms) of each hotel is perishable on each day. Thus, a good pricing policy can benefit the matching of supply and demand, and improve the overall revenue. In practice, most pricing strategies recommend an optimal price to maximize the revenue based on a \textit{demand curve} \cite{dynamicPricing2015} that depicts the relationship between the price of a room and the demanded rooms, or particularly referred to as \emph{occupancy}, at that price. Therefore, occupancy estimation is the key to the success of dynamic pricing. 

However, an accurate occupancy estimate is challenging as the demand curve exhibits different patterns over time due to the diversity in hotel characteristics and external influences such as events, seasonality, \etc\
Regression models are widely adopted in existing works for occupancy prediction. For example, Ye \etal ~\cite{customized2018} use a Gradient Boosting Machine (GBM) ~\cite{friedman2001greedy} to map a set of raw features to an estimated booking probability for Airbnb's listings. Zhang \etal ~\cite{deeplearningHotel2019} capitalize on a seq2seq model \cite{sutskever2014sequence} to predict the future occupancy based on the hotel features and statistics. However, these regression models may suffer from the \textit{data sparseness} as many rooms only have reservations on certain days while the reservation prices are generally in a narrow range, and \textit{endogeneity problem}~\cite{econometrics2008} as many features are price dependent (\eg, the feature of historical sales is positively correlated with price). 
To address this, in this paper, we aim at a more accurate and explainable occupancy prediction approach for dynamic hotel pricing.
% that address these issues of existing works.


\begin{comment}
Ye \etal ~\cite{customized2018} 
%recognize the ``time-varying" and ``listing-varying" properties of demand at Airbnb,
propose to predict the booking probability of listing night at Airbnb and suggest the optimal price with a demand-enhanced pricing model, which is \zemin{only} customized for Airbnb's unique listings and cannot be adapted to general hotel pricing with multiple \zemin{inventories}. 
Zhang \etal ~\cite{deeplearningHotel2019} capitalize on a seq2seq model \cite{sutskever2014sequence} to predict the future occupancy based on the hotel features and statistics, and regress the suggested price with a DNN model~\cite{nielsen2015neural}. However, the regression model may suffer from the problem of \textit{endogeneity}~\cite{econometrics2008} as many features are price dependent (\eg, the feature of historical sales is positively correlated with price). 
\end{comment}

%as the demand is influenced by a series of complex factors including events, seasonality \etc\, and thus is changing over time and exhibits different patterns. Meanwhile, these complex factors also make it challenging to estimate the demanded rooms \zemin{in a certain hotel} on a given night, or particularly referred to as \emph{occupancy estimation}.  

%In practice, most pricing strategies propose to recommend an optimal price to maximize the revenue based on a \textit{demand curve}~\cite{dynamicPricing2015} that depicts the relationship between the price of a product and the expected demand at that price. Therefore, how to accurately estimate the demand function is the key to the success of dynamic pricing. 

%Specifically, a demand curve depicts the relationship between the price of a product and the demanded quantity of the product at that price. Given a demand curve $F(P)$ that denotes demands as the function of price $P$, the optimal price is simply the one yields maximal $P\times F(P)$.

%is a common practice, 
%estimating the demand function is not trivial as the the number of demanded rooms \zemin{in a certain hotel} on a given night,
%or particularly referred to as \emph{occupancy}, is influenced by %\zemin{a series of} 
%complex factors such as hotel popularity, seasonality, competitor prices, \etc\


\stitle{Motivation.} Our idea is inspired by the concept of ``price elasticity" in economics~\cite{econometrics2008}. Particularly, we observe that though price is a significant affecting factor for hotel occupancy (\eg, the more a hotel lowers the price, the higher the occupancy rate), the sensitivity of occupancy to price change (or price elasticity of demand) could be quite different. 
\textit{On the one hand}, the price elasticity of hotels with different characteristics is essentially different, \eg, the occupancy of luxury hotels are less price-sensitive than budget hotels as they have less substitutes in the market place. 
\textit{On the other hand}, even for a same hotel room, its price elasticity could be varying across time due to the external factors such as seasonality and market trend. For example, hot spring hotels are less price-sensitive in winter as the demand is seasonal. 
\textit{Moreover}, the price elasticity of hotels in a shared market synchronously fluctuates due to the competition among them. For example, discount on a hotel room would drive higher demand for it, and at the same time lead to the lower occupancy for its competitors.

%with a novel \textit{elastic demand function} that explicit , and a price elastic prediction model 

%investigate the factors that affecting the occupancy of hotel rooms for more accurate and explainable occupancy prediction. 
%Our idea is inspired by the concept of ``price elasticity" in microeconomics~\cite{econometrics2008} that explains the relationship between a product's price and demand for that product. In particular, 
%Machine learning techniques are widely used for occupancy estimation in existing works on hotel pricing. For example, Ye \etal ~\cite{customized2018} propose to use a gradient boosting machine to learn the booking probability of listing night at Airbnb, and predict the ``optimal price" with a regression model. Zhang \etal ~\cite{deeplearningHotel2019} apply a seq2seq model to predict the future occupancy based on hotel features and statistics and regress the suggested price with a DNN model. However, these studies ignore the problem of \textit{endogeneity}, that is, selling price is the endogenous variable that correlated with the other features in the regression model. To solve this problem, in this paper, we try to directly model the effects of price and input features on the occupancy rather than learning the price from features. 

\stitle{Proposal.} Such observations motivate us to explicitly model the \textit{price elasticity} of demand in occupancy estimation. Specifically, we define the occupancy of a hotel room as a function $F(P,\beta)$ of its selling price $P$ and the price elasticity coefficient $\beta$, and propose a price elasticity model (PEM) to learn the dynamic price elasticity coefficient in the occupancy function. Once $\beta$ is inferred, the optimal price can be easily obtained based on the demand curve $F(P,\beta)$.

In addition to better modeling the demand dynamics, the elastic demand function brings two other advantages: 
1) the price elasticity of rooms are inherently similar to the price elasticity of hotels they belong to. Thus, the hotel-level reservation data can be used to handle the data sparsity issue and enhance the model training; 2) the features affecting $\beta$ are less dependent on price but more relevant to the room characteristics and external influences. Thus, it is promising to alleviate the endogeneity problem with proper model design.

Specifically, we comprehensively examine the features affecting the price elasticity and identify three orthogonal groups of factors: \textit{competitive factors} (\ie, the influence of competitive hotels in a same market), \textit{temporal factors} (\ie, the effect of hotel popularity and market trend), and \textit{characteristic factors} (\ie, the effect of basic features). We develop a competitiveness representation module and a multi-sequence fusion module to capture the competitive factors and the temporal factors, and attentively integrate them for occupancy prediction. Our model is trained in a multi-task learning framework using hotel occupancy prediction task to assist room occupancy prediction, to handle the data sparsity issue. 
%The representations are later integrated with the characteristics factor 

%and an attentive prediction module, with each capturing one type of factor to alleviate .
 
 

%The price elasticity model consists of 1) a competitiveness representation module to , 2), and 3) a prediction module that integrates the competitive factors and temporal factors with the basic features (\ie, the characteristic factors) and real-time information to predict the price elasticity. To handle the data sparsity, we  in a multi-task training framework.

% In summary, our main contributions are three-fold. 
% (1) We propose a novel demand function that explicitly model the price elasticity of demand for hotel dynamic pricing.
% (2) We identify different types of factors affecting the price elasticity and design a price elasticity learning network to capture those factors for room-level and hotel-level price elasticity prediction.
% (3) We conduct extensive experiments on real-world datasets and validate the superiority of our method for both occupancy prediction and dynamic pricing.

% Our main contributions are summarized as follows: 1) We are the first to formally define and utilize the price elasticity of demand to enhance the accuracy of occupancy estimation in hotel dynamic pricing. 2) We propose a multi-task price elasticity learning framework that tackles the data sparsity using hotel-level occupancy prediction to assit the room-level occupancy, and alleviate the endogeneity problem with three carefully desgined modules. 3) We conduct extensive experiments on two real-world datasets and validate the superiority of our method for both occupancy prediction and dynamic pricing.

\stitle{Contributions.} Our contributions are three-fold. (1) We propose to utilize the price elasticity of demand to enhance the occupancy estimation and formally define a novel elastic demand function for hotel dynamic pricing. 
% (2) We propose a multi-task price elasticity learning framework that tackles the data sparsity using hotel-level occupancy prediction to assist the room-level occupancy, 
(2) We develop a multi-task price elasticity learning framework that tackles the data sparsity of room-level occupancy with the assistance of hotel-level occupancy prediction, and alleviate the endogeneity problem with carefully designed modules. 
% (3) We conduct extensive experiments on two real-world datasets and validate the superiority of our method for both occupancy prediction and dynamic pricing.
(3) Extensive experiments on two real-world datasets validate the superiority of our method for both occupancy prediction and dynamic pricing.


%learn the competitiveness of each selling price in a competing group of hotels (\ie, captures the competitive factors affecting price elasticity), and 2) multi-sequence fusion module to earns a temporal popularity representation based on multiple sequences of time-varying features such as sales statistics

%a xxx module that captures the influence of competitive hotels in a same market (\ie, the competitive factors), a xxx module that captures the effect of hotel popularity and market trend (\ie, the time-varying factors), and a feature embedding layer to infuse the effect of the side information and real-time features (\ie, the room-night varying factors). To handle the data sparsity, we use the hotel-level occupancy prediction task to assist room-level occupancy prediction in a multi-task training framework.
%train the model in a multi-task learning framework where the hotel-level occupancy prediction is used to assist room-level occupancy prediction.


%Such observation motivates us to explicitly model the \textit{price elasticity}, a economic notion that measures the influence of price change on the demand of the products offered, of a hotel/room in occupancy rate estimation. Once $\beta$ is predicted, the optimal price can be obtained by maximizing the 




==> sec-model.tex <==
\section{Approach}
\label{sec:model}
In this section, we define a novel demand function in hotel dynamic pricing, and present the proposed price elasticity learning model.
\subsection{Elastic Demand Function}
\label{subsec:problem}
In online hotel booking platform, a typical hotel provides multiple types of rooms for reservation on each day. The demand or occupancy of rooms varies across room-types (\eg, luxury rooms, economic rooms) and changes over time (\eg, weekday, weekend). 

% To forecast the occupancy $O_i^t$ of a room type $r_i$ on a specific night $t$, as motivated in Sect.~\ref{sec:intro}, we propose to model $O_i^t$ as a function of the selling price $P_i^t$ and price elasticity coefficient $\beta_i^t$. We now concretely define the demand function based on two intuitions: 1) changes in $O_i^t$ are inversely related to changes in $P_i^t$ (\eg, demand usually falls when price rises); 2) how much $O_i^t$ changes is regulated by the price elasticity coefficient $\beta_i^t$.

To forecast the occupancy $O_r^t$ of a room type $r$ on a specific night $t$, as motivated in Sect.~\ref{sec:intro}, we propose to model $O_r^t$ as a function of the selling price $P_r^t$ and price elasticity coefficient $\beta_r^t$. We now concretely define the demand function based on two intuitions: 1) changes in $O_r^t$ are inversely related to changes in $P_r^t$ (\eg, demand usually falls when price rises); 2) how much $O_r^t$ changes is regulated by the price elasticity coefficient $\beta_r^t$.
% Based on these intuitions, 
Therefore, we can formalize the demand function in a concise yet effective way as
% and our demand function for occupancy prediction can be formalized as:
\begin{equation}
\vspace{-1mm}
    O_r^t= \bar{O}_r \cdot (P_r^t/\bar{P}_r)^{-\beta_r^t},
\label{eq:demand}
\end{equation}
%\vspace{-1mm}
% \begin{equation}
%     O_i^t= \bar{O}_i \cdot (P_i^t/\bar{P}_i)^{-\beta_i^t},
% \label{eq:demand}
% \end{equation}
% where $\bar{O}_i$ and $\bar{P}_i$ is the constant benchmark occupancy and price, respectively, \eg, average occupancy or price in one week.
where $\bar{O}_r$ and $\bar{P}_r$ are the constant benchmark occupancy and price, respectively, \eg, the average occupancy or price in one week.
%where $\beta_r^t\in\mathbb{R}$ is the learnable price elasticity coefficient. 

%In Eq.~\eqref{eq:demand}, $\bar{O}_r$ and $\bar{P}_r$ can be obtained from the statistics, and $\beta_r^t$, the key to the success of occupancy prediction, can be learned with a price elasticity model which will be discussed in Sect.~\ref{subsec:PEM}. 

Therefore, $\beta_r^t$ is the key to the success of occupancy prediction. Once $\beta_r^t$ is inferred, we can simply sample a set of prices $P_r^t$ in a reasonable range to calculate the corresponding $O_r^t$, and the optimal price is the one that maximizes the expected revenue
% \begin{equation}
%      P_i^{t*} = \arg \max_{P_i^t} (P_i^t-P_i^0) \cdot O_i^t,
% \end{equation}
\begin{equation}
\vspace{-2mm}
     P_r^{t*} = \arg \max_{P_r^t} (P_r^t-P_r^0) \cdot O_r^t,
\end{equation}
\vspace{-1.5mm}
where $P_r^0$ is the cost price of room type $r$.

%\sstitle{Dynamic pricing with occupancy estimation.}
 %Due to the uncertainty of demand on each night, the optimal prices for each type of rooms change over time. 
\begin{comment}

Dynamic pricing is a pricing strategy that recommends an optimal price for each room-night to maximize the revenue.

Let $H$ denote a set of hotels. For each hotel $h\in H$, the set of different rooms provided by $h$ is denoted as
% $R^h=\{r_1^h, r_2^h, \ldots\}$, 
$R^h=\{R^h_{r_1}, R^h_{r_2}, \ldots\}$, 
where $R^h_{r_i}$ refers to the set of rooms belonging to room type $r_i$ in hotel $h$ (\ie, each room type has multiple inventories). 
The demand or occupancy of a room type $i$ on a specific night $t$ can be calculated with the concrete values of $\bar{O}_i^t$, $\bar{P}_i^t$ and $\beta_i^t$. Note that, we omit $h$ in the superscript to simplify the notations when $h$ is clarified in the context.
The optimal price for room type $i$ is the one that maximizes the overall revenue,
\begin{equation}
    P_i^{t*} = \arg \max_{P_i^t} (P_i^t-P_i^0) \cdot \bar{O}_i^t \cdot (P_i^t/\bar{P}_i^t)^{-\beta_i^t}.
\label{eq:price}
\end{equation}
In this equation, $P_i^0$ is the cost price of $r_i$, 


\end{comment}


\subsection{Price Elasticity Prediction Model}
\label{subsec:PEM}
We now present the \textbf{P}rice \textbf{E}lasticity prediction \textbf{M}odel (PEM) to learn the price elasticity coefficient $\beta_r^t$ in Eq.~\eqref{eq:demand}. We identify three types of factors affecting the price elasticity in the hotel market:
% and the PEM model is designed to capture these factors accordingly.
% \begin{itemize}[leftmargin=*]
%     \item \emph{Competitive factors}: the external affecting factors in a competitive environment, such as the price and quality of competitors. For example, hotels with more substitutes are usually more sensitive to price change, while hotels which are more competitive than the substitutes are less price-elastic.
%     \item \emph{Temporal factors}: the time-varying factors which relate to specific scenarios such as events, seasonality, popularity, \etc\ For example, the price elasticity of hot spring hotels are quite different in winter and summer as a hotel usually reacts differently to price changes when its popularity increases or decreases. 
%     \item \emph{Characteristic factors}: the internal factors which relate with the basic features of hotels or rooms, such as hotel star, location and business district. Hotels with different characteristics naturally have different price elasticity. 
% \end{itemize}
(1) \emph{Competitive factors} such as the price and quality of competitors. For example, hotels that have better quality than its competitors are less price-elastic.
(2) \emph{Temporal factors} such as events, seasonality, popularity, \etc\ For example, the price elasticity of hot spring hotels are quite different in winter and summer due to the seasonal increase or decrease of its popularity. 
(3) \emph{Characteristic factors} such as hotel star, location and business district. Hotels with different characteristics naturally have different price elasticity. 

Our PEM model is designed to leverage all these factors for dynamic demand learning. As shown in Fig.~\ref{fig:archi}, PEM is developed in a multi-task learning framework that simultaneously predicts the price elasticity coefficient $\beta_r^t$ of a room $r$ and the price elasticity coefficient $\beta_h^t$ of its belonging hotel $h$ at night $t$. For each prediction task, the input contains the aforementioned features, as well as the contextual features such as real-time price, holiday-or-not information. 
%The statistical features (\eg, ) of a hotel are the aggregated
To alleviate the endogeneity problem, the basic features of location, hotel star \etc\ and contextual features are transformed into low-dimensional representations through an embedding layer, while the other features related to competitive factors and temporal factors are respectively processed with two sub-modules: Competitiveness Representation Module (CRM) and Multi-Sequence Fusion Module (MSFM), elaborated in the following subsections. Note that, we describe these modules in the context of room-level prediction task while for group-level task we only explain the specific inputs. 

% As discussed in Sect.~\ref{sec:intro}, 
%In particular, the hotel price elasticity prediction can assist the main task to address the data sparsity issue and enhance the model training.

%We adopt the multi-task framework for two reasons: 1) the room reservation data are much sparse than hotel reservation data (\ie, many rooms in a hotel may not be reserved on certain night); 2) the price elasticity of rooms is inherently similar to the price elasticity of hotels. Therefore, 

\begin{figure*}
    \centering
    \vspace{-2mm}
    \includegraphics[width=0.85\textwidth]{samples/framework_v3.pdf}
    \vspace{-3mm}
    \caption{The proposed PEM model for price elasticity prediction.}
    \label{fig:archi}
    \vspace{-2mm}
\end{figure*}

%These two types of price elasticity are similarly modeled with

%Since these modules of room- and hotel-level prediction have the same structure, we will focus on the room price elasticity prediction in the following discussion.

%1) a \emph{Competitiveness Representation Module (CRM)} that takes the features of competing rooms and price of specific room-night as input and learns a competitiveness vector for that price on a room-price graph constructed from the reservation statistics of competing rooms; 2) a \emph{Multi-Sequence Fusion Module (MSFM)} that learns a temporal popularity representation based on multiple sequences of time-varying features such as sales statistics, historical prices. These representations are attentively aggregated for occupancy estimation. 
%an \emph{integrated predicting module} that incorporates the two vectors with the characteristic features to predict the price elasticity. The integrated prediction module for room price elasticity prediction also takes the intermediate output of hotel price elasticity representation as input to predicate room price elasticity. 
%We will discuss the details of each module next. 

%In the following discussion, we only focus on the modules for room price elasticity prediction while those for hotels are generally the same.


%Since the modules of room- and hotel-level prediction have the same structure, we will focus on the room price elasticity prediction in the following discussion.
%As room-level reservation data are much sparse, but the price elasticity of rooms are inherently similar to the price elasticity of hotels, we design a multi-task learning framework to simultaneously train the model with room price elasticity prediction and hotel price elasticity prediction. These two types of price elasticity are similarly modeled except that the integrated prediction module for room price elasticity prediction would also take the intermediate output of hotel price elasticity. We will discuss the details of each module next.
\subsubsection{Competitiveness Representation Module.} As discussed, the price elasticity of rooms in a shared market synchronously fluctuates due to the competition among them. 
% We design this module to learn the competitiveness of each selling price among a group of similar/competing rooms. 
To model this pattern, we propose the CRM module (Fig.~\ref{fig:archi}(b)) to learn the competitiveness of each selling price among a group of similar/competing rooms. The input of CRM consists of the basic features of all rooms $R$ (or hotels $H$), a specific room-type $r$  and the selling price $P_r^t$. 

%\sstitle{Identifying competing group.} 
To identify the competing groups, we cluster the rooms based on their basic features such as location, hotel star, and business district, with $K$-means clustering algorithm ($K$ equals to the number of business districts). The rooms in each cluster have similar qualities and usually compete with each other in the shared market, and thus the price change of one room would affect the others. 
For each group, we construct a heterogeneous room-price graph with two types of nodes, \ie, price and room, based on the reservation data in recent $30$ days. Each edge between a room node and a price node is weighted, indicating how many times the room was reserved at the connecting price. For each specific price, as its connections to rooms are sparse, we group the continuous price into several intervals (\eg, \$100-\$150, \$150-\$200) and represent each price interval with one single node.
% As the connections between room and each specific price are sparse, we set several range (\eg, \$100-\$150, \$150-\$200) and represent the prices falling in a same range with one single node.

%\sstitle{Modeling price competitiveness.} 
From the constructed room-price graph, we conclude two intuitions:
1) Rooms that are frequently connected by the same price nodes are more similar in price-competitiveness
(\ie, they are better substitutes for each other);
2) Prices with more connections to the same rooms 
are more competitive than those have fewer connections.
Thus, we apply metapath2vec~\cite{metapath2vec2017} with metapaths \textit{room-price-room} and \textit{price-room-price}, to capture the above semantics and generate the embeddings for room and price nodes. %\zeminC{self-supervised loss.}
% 
%Given the selling price $P_r^t$ of a room $r$ on night $t$, if $P_r^t$ is modeled in the room-price graph, we can directly obtain the competitiveness representation $\mathbf{c}_r^t$ of $P_r^t$. While if $P_r^t$ does not match any price nodes, we locate two most similar prices in the graph, and use the average of their embeddings to represent $\mathbf{c}_r^t$.
Given the input selling price $P_r^t$, we can retrieve its competitiveness representation $\vp{r}{t}$ from the price embeddings, or average the representations of the two most similar price nodes if $P_r^t$ does not match any price node in the graph.
\subsubsection{Multi-sequence fusion module.}
The multi-sequence fusion model (Fig.~\ref{fig:archi}(c)) is designed to model the temporal factors that affect the price elasticity. The input of this module consists of the sequence of daily clicks (\ie, number of users who clicks the room), sequence of daily searches (\ie, number of searches for the room), and sequence of historical booking prices, of room-type $r$ in the latest $30$ days. For hotel-level task, the input statistics are the sum of all room statistics in a hotel.
%which reflect its recent popularity.
\begin{comment}
In particular, we take several value sequences as input, \ie, 
sequence of sales $\mathcal{S}_{i}=(\ldots, s_i^t,\ldots)$, sequence of clicks \zemin{(\ie, number of users who clicks the room)} $\mathcal{C}_i=(\ldots, c_{i}^t,\ldots)$, sequence of searches \zemin{(\ie, number of searches for the room)} $\mathcal{E}_{i}=(\ldots, e_{i}^t,\ldots)$, and sequence of booking price $\mathcal{B}_{i}=(\ldots, b_{i}^t,\ldots)$ on each night $t$.
\end{comment}
% \zemin{Note that, each value in these sequences denotes the corresponding operation number in that day.}
% \zeminC{seq长度是month，将他们concate组成matrix。}

As shown in Fig.~\ref{fig:archi}(c), the multiple sequences are fused with a two-layer Bi-GRU \cite{traffic2020} to model the combination of features and thus capture the popularity trends. 
% We also apply two one-dimensional convolutions with different kernel sizes to capture the combined features of multiple sequences and explore the local patterns from them. 
We also apply two one-dimensional convolutions with different kernel sizes followed with an average pooling operation, to exploit the underlying local patterns for all the sequences.
The representations of popularity trends and local patterns are then concatenated as the final temporal vector ${m}_r^t$ .
\subsubsection{Multi-task losses.}
The competitiveness and temporal vectors are further employed to form a multi-task loss involving room-level and hotel-level price elasticity predictions for end-to-end training.
% The competitiveness and temporal vectors can be further fed into the task losses for both room- and hotel-levels for end-to-end training, as shown in Fig.~\ref{fig:archi}(a). 
For room-level task, we concatenate both the competitiveness and temporal vectors $m_r^t||c_r^t$, as well as the contextual and basic room features, to form a unified feature representation, which is further fed into two fully-connected layers to estimate the price elasticity. We also leverage the intermediate representations of hotel-level features $X_h^t$ in room-level prediction by a gating mechanism based on the similarity of their popularity representations $m_r^t \cdot m_h^t$. The intuition is that the price elasticity of hotels will have more influence on rooms with similar popularity. 
For hotel-level task, $c_h^t$ and $m_h^t$ are concatenated and fed into an MLP to predict $\beta_h^t$. Finally, the estimated room occupancy $O_r^t$ and hotel occupancy $O_h^t$ can be derived by Eq.~\eqref{eq:demand}.
%Therefore, based on Eq.~\eqref{eq:demand}, we can predict the occupancy of room $r$ on night $t$ as $\hat{O}_r^t=\bar{O}_r^t(P_r^t/\bar{P}_r^t)^{-\beta_r^t}$.

% Finally, the competitiveness vector and temporal vector are concatenated with the embeddings of room basic features, which is further fed to two fully-connected layers, along with the intermediate representation of hotel-level task, to generate the price elasticity $\beta_r^t$. Based on which, the occupancy of room $r$ on night $t$ can be predicated using Eq.~\ref{eq:demand}: $\hat{O}_r^t=\bar{O}_r^t(P_r^t/\bar{P}_r^t)^{-\beta_r^t}$.
%The intermediate representation of hotel-level task is also transferred to the FC layer to improve the room price elasticity prediction.


% Our PEM model is trained in the multi-task framework for room and hotel price elasticity prediction, with the objective of minimizing the total loss of these two tasks.

For model training, given $n$ selling price and occupancy tuples of historical room-level transactions $T_r=\{P_{ri}^t, O_{ri}^t\}_{i=1}^n$, 
% Given $n$ training samples of selling price and occupancy from historical room-level transactions $T_r=\{P_{ri}^t, O_{ri}^t\}_{i=1}^n$, 
and $m$ tuples of hotel-level transactions $T_h=\{P_{hj}^t, O_{hj}^t\}_{j=1}^m$ where $P_{h*}$ (or $O_{h*}$) is the sum of price (or occupancy) over all rooms in hotel $h$, we construct the overall loss by combining the room-level prediction loss $H_\delta(O_{ri}^t, \hat{O}_{ri}^t)$ and hotel-level prediction loss $H_\delta (O_{hj}^t, \hat{O}_{hj}^t)$:
\begin{equation}
\vspace{-2mm}
  \mathcal{L}=\lambda \sum_{i=1}^n H_\delta(O_{ri}^t, \hat{O}_{ri}^t) + (1-\lambda) \sum_{j=1}^m H_\delta (O_{hj}^t, \hat{O}_{hj}^t),
    \label{eq:loss}
\end{equation}
where $\lambda$ is a hyper-parameter to balance two tasks, and each prediction loss $H_\delta(y,\hat{y})$ is defined as the huber loss~\cite{Robust1964} with hyperparameter $\delta\in R^+$:
\begin{equation}
H_\delta (y,\hat{y})= \begin{cases}
\frac{1}{2} (y-\hat{y})^2, &  \text{if} \quad(y-\hat{y})\leq \delta; \\
\delta (y-\hat{y}) -\frac{1}{2}\delta^2, & \text{otherwise}.
\end{cases}
\end{equation}

==> sec-related_work.tex <==
\section{Related work}
\label{sec:related}
Dynamic pricing has been extensively studied and widely used in various businesses \cite{ct21} where selling prices of products or services are dynamically adjusted based on the price-demand relations. 
Given a demand function $F(P)$ (or demand curve) that evaluates how demand varies with respect to price, the optimal price $P$ can be obtained by maximizing the expected revenue $F\times F(P)$ \cite{ct7,ct19,ct20,ct27,ct40,ct41,ct42,ct43}. 

Some early works propose to learn the unknown parameters of the demand function within a Bayesian framework, while a major disadvantage of which is the computational intractability of the optimal solution. In practice, non-parametric methods are frequently used in demand estimation.   


%The topic of dynamic pricing has received a considerable amount of attention in recent years \cite{ct21,ct23,ct24,ct15,ct29,ct30}. Most studies try to obtain the optimal price via maximizing the expected revenue based on the estimated demand curve \cite{ct7,ct19,ct20,ct27,ct40,ct41,ct42,ct43} in various fields. Due to the demand function changes according to circumstances, researchers often introduce a variety of factors, such as reference prices \cite{ct40,ct41} and the amount of cumulative sales \cite{ct43} for better demand estimation. In order to learn the demand function whose parameters may change over time, some researchers adopt machine learning techniques such as parametric approach \cite{ct46,ct47} using classical maximum likelihood or least-squares estimators, Markov chain Monte Carlo \cite{ct48} and bayesian approaches \cite{ct44,ct45}. 

Machine-learning based approaches are capable of modeling multiple factors that influence the demand in different areas \cite{ct21}.
%Moreover, some scholars propose other dynamic pricing strategies. 
For example, Rana \textit{et al.} \cite{ct49} adopt reinforcement learning algorithms to analyze how firms can both learn and optimize their pricing strategies while interacting with their customers. Chen \textit{et al.} \cite{ct50} propose a novel Dynamic Pricing Strategy (DPS) in traffic-aware road networks. Recently, Shukla \textit{et al.} \cite{ct23} present a multi-stage pricing strategy, which developed a pricing model that provides dynamic pricing recommendations specific to each customer interaction and optimizes expected revenue per customer. However, the above dynamic pricing research works in other fields cannot be applied to hotel pricing due to the uniqueness of industry characteristics.  
For example, the method developed in \cite{ct23} is not applicable to hotel pricing because of all the customers in hotel pricing scenario are identical.


As for hotel dynamic pricing, most researchers applied machine learning algorithms to model hotel reservation probability \cite{ct24,ct15,ct29,ct30} and used regression model to predict the optimal price in the future. For example, Ye \textit{et al.}~\cite{ct15} propose a hotel pricing model customized for Airbnb shared homes, which can not be generalized to other hotel dynamic pricing scenarios. Zhang \textit{et al.} \cite{ct24} transform pricing problem into the regression problem of hotel price, which takes the estimated occupancy rate as the input of the pricing model. However, the impact of occupancy rate in the pricing model is less significant, and the method of price regression can not solve the problem of endogenous variables \cite{ct28}. In addition, these pricing strategies ignored the hotel characteristics of popularity and competitiveness.
% bayesian approaches were widely used by Qu \textit{et al.} \cite{ct44} and Kwon \textit{et al.} \cite{ct45}, and Boer \textit{et al.} \cite{ct46} and Keskin \textit{et al.} \cite{ct47} taked a parametric approach, . Moreover, Do Chung \textit{et al.} \cite{ct48} developed a demand learning algorithm using Markov chain Monte Carlo methods to estimate model parameters. 


% While 
% Most of the previous studies focus on the accuracy of demand estimation, which aims to maximize revenue through demand based variable pricing (demand forecast based on each future date). However, it is aimed to get an accurate demand curve is extremely difficult.
% In summary, the existing dynamic pricing methods either ignore the characteristics of hotel, or the pricing strategy is non-universal. In this paper, we propose a novel dynamic pricing strategy to alleviate these problems. Three modules with the pricing characteristics of the hotel are developed to capture the long short-term popularity and competitiveness. And directly output the optimal price via our model. 
